MITHRIL: Mining Sporadic Associations for Cache Prefetching

The growing pressure on cloud application scalability has accentuated storage performance as a critical bottle- neck. Although cache replacement algorithms have been extensively studied, cache prefetching - reducing latency by retrieving items before they are actually requested remains an underexplored area. Existing approaches to history-based prefetching, in particular, provide too few benefits for real systems for the resources they cost. We propose MITHRIL, a prefetching layer that efficiently exploits historical patterns in cache request associations. MITHRIL is inspired by sporadic association rule mining and only relies on the timestamps of requests. Through evaluation of 135 block-storage traces, we show that MITHRIL is effective, giving an average of a 55% hit ratio increase over LRU and PROBABILITY GRAPH, a 36% hit ratio gain over AMP at reasonable cost. We further show that MITHRIL can supplement any cache replacement algorithm and be readily integrated into existing systems. Furthermore, we demonstrate the improvement comes from MITHRIL being able to capture mid-frequency blocks.

==> ref <==
@inproceedings{patterson95,
 author = {Patterson, R. H. and Gibson, G. A. and Ginting, E. and Stodolsky, D. and Zelenka, J.},
 title = {Informed Prefetching and Caching},
 booktitle = {Proceedings of the Fifteenth ACM Symposium on Operating Systems Principles},
 series = {SOSP '95},
 year = {1995},
 isbn = {0-89791-715-4},
 location = {Copper Mountain, Colorado, USA},
 pages = {79--95},
 numpages = {17},
 url = {http://doi.acm.org/10.1145/224056.224064},
 doi = {10.1145/224056.224064},
 acmid = {224064},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{kaplan02,
 author = {Kaplan, Scott F. and McGeoch, Lyle A. and Cole, Megan F.},
 title = {Adaptive Caching for Demand Prepaging},
 booktitle = {Proceedings of the 3rd International Symposium on Memory Management},
 series = {ISMM '02},
 year = {2002},
 isbn = {1-58113-539-4},
 location = {Berlin, Germany},
 pages = {114--126},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/512429.512445},
 doi = {10.1145/512429.512445},
 acmid = {512445},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {adaptive caching, block paging, clustering, prepaging},
} 


@article{wu2009sequential,
    title={Sequential file prefetching in Linux},
    author={Wu, Fengguang},
    journal={Advanced Operating Systems and Kernel Applications: Techniques and Technologies: Techniques and Technologies},
    pages={218},
    year={2009},
    publisher={IGI Global}
}


@article{McKusick1984FFS,
    author = {McKusick, Marshall K. and Joy, William N. and Leffler, Samuel J. and Fabry, Robert S.},
    title = {A Fast File System for UNIX},
    journal = {ACM Trans. Comput. Syst.},
    issue_date = {Aug. 1984},
    volume = {2},
    number = {3},
    month = aug,
    year = {1984},
    issn = {0734-2071},
    pages = {181--197},
    numpages = {17},
    url = {http://doi.acm.org/10.1145/989.990},
    doi = {10.1145/989.990},
    acmid = {990},
    publisher = {ACM},
    address = {New York, NY, USA},
    keywords = {UNIX, application program interface, file system design, file system organization, file system performance},
} 

@inproceedings{Baker1991MDF,
 author = {Baker, Mary G. and Hartman, John H. and Kupfer, Michael D. and Shirriff, Ken W. and Ousterhout, John K.},
 title = {Measurements of a Distributed File System},
 booktitle = {Proceedings of the Thirteenth ACM Symposium on Operating Systems Principles},
 series = {SOSP '91},
 year = {1991},
 isbn = {0-89791-447-3},
 location = {Pacific Grove, California, USA},
 pages = {198--212},
 numpages = {15},
 url = {http://doi.acm.org/10.1145/121132.121164},
 doi = {10.1145/121132.121164},
 acmid = {121164},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@article{Teng1984MID,
 author = {Teng, J. Z. and Gumaer, R. A.},
 title = {Managing IBM Database 2 Buffers to Maximize Performance},
 journal = {IBM Syst. J.},
 issue_date = {June 1984},
 volume = {23},
 number = {2},
 month = jun,
 year = {1984},
 issn = {0018-8670},
 pages = {211--218},
 numpages = {8},
 url = {http://dx.doi.org/10.1147/sj.232.0211},
 doi = {10.1147/sj.232.0211},
 acmid = {1663500},
 publisher = {IBM Corp.},
 address = {Riverton, NJ, USA},
} 


@inproceedings{gill2007amp,
    title={{AMP}: adaptive multi-stream prefetching in a shared cache},
    author={Gill, Binny S and Bathen, Luis Angel D},
    booktitle={Proceedings of the 5th USENIX conference on File and Storage Technologies},
    pages={26--26},
    year={2007},
    organization={USENIX Association}
}

@inproceedings{gill2005sarc,
    title={{SARC}: Sequential Prefetching in Adaptive Replacement Cache.},
    author={Gill, Binny S and Modha, Dharmendra S},
    booktitle={USENIX Annual Technical Conference, General Track},
    pages={293--308},
    year={2005}
}

@inproceedings{li2008tap,
    title={{TaP}: table-based prefetching for storage caches},
    author={Li, Mingju and Varki, Elizabeth and Bhatia, Swapnil and Merchant, Arif},
    booktitle={Proceedings of the 6th USENIX Conference on File and Storage Technologies},
    pages={6},
    year={2008},
    organization={USENIX Association}
}

@inproceedings{soundararajan2008quickmine,
    title={Context-Aware Prefetching at the Storage Server.},
    author={Soundararajan, Gokul and Mihailescu, Madalin and Amza, Cristiana},
    booktitle={USENIX Annual Technical Conference},
    pages={377--390},
    year={2008}
}

@inproceedings{ding2007diskseen,
    title={DiskSeen: Exploiting Disk Layout and Access History to Enhance I/O Prefetch.},
    author={Ding, Xiaoning and Jiang, Song and Chen, Feng and Davis, Kei and Zhang, Xiaodong},
    booktitle={USENIX Annual Technical Conference},
    volume={7},
    pages={261--274},
    year={2007}
}

@article{nanopoulos2003data,
    title={A data mining algorithm for generalized web prefetching},
    author={Nanopoulos, Alexandros and Katsaros, Dimitrios and Manolopoulos, Yannis},
    journal={IEEE transactions on knowledge and data engineering},
    volume={15},
    number={5},
    pages={1155--1169},
    year={2003},
    publisher={IEEE}
}

@inproceedings{chen2010adaptive,
    title={An adaptive data prefetcher for high-performance processors},
    author={Chen, Yong and Zhu, Huaiyu and Sun, Xian-He},
    booktitle={Cluster, Cloud and Grid Computing (CCGrid), 2010 10th IEEE/ACM International Conference on},
    pages={155--164},
    year={2010},
    organization={IEEE}
}


@inproceedings{yang2016tombolo,
    title={Tombolo: Performance Enhancements for Cloud Storage Gateways},
    author={Yang, Suli and Srinivasan, Kiran and Udayashankar, Kishore and Krishnan, Swetha and Feng, Jingxin and Zhang, Yupu and Arpaci-Dusseau, Andrea C and Arpaci-Dusseau, Remzi H},
    booktitle={IEEE 32nd Symposium on Mass Storage Systems and Technologies, MSST 2016},
    year={2016}
}

@inproceedings{lin2008amp,
    title={{AMP}: an affinity-based metadata prefetching scheme in large-scale distributed storage systems},
    author={Lin, Lin and Li, Xuemin and Jiang, Hong and Zhu, Yifeng and Tian, Lei},
    booktitle={Cluster Computing and the Grid, 2008. CCGRID'08. 8th IEEE International Symposium on},
    pages={459--466},
    year={2008},
    organization={IEEE}
}

@inproceedings{lei1997analytical,
    title={An analytical approach to file prefetching},
    author={Lei, Hui and Duchamp, Dan},
    booktitle={USENIX Annual Technical Conference},
    pages={275--288},
    year={1997}
}

@article{jiang2013prefetching,
    title={A prefetching scheme exploiting both data layout and access history on disk},
    author={Jiang, Song and Ding, Xiaoning and Xu, Yuehai and Davis, Kei},
    journal={ACM Transactions on Storage (TOS)},
    volume={9},
    number={3},
    pages={10},
    year={2013},
    publisher={ACM}
}

@inproceedings{li2012real,
    title={Real-time Data Prefetching Algorithm Based on Sequential Patternmining in Cloud Environment},
    author={Li, Jiazheng and Wu, Shaochun},
    booktitle={Industrial Control and Electronics Engineering (ICICEE), 2012 International Conference on},
    pages={1044--1048},
    year={2012},
    organization={IEEE}
}


@inproceedings{li2004cminer,
    title={{C-Miner}: Mining Block Correlations in Storage Systems.},
    author={Li, Zhenmin and Chen, Zhifeng and Srinivasan, Sudarshan M and Zhou, Yuanyuan},
    booktitle={FAST},
    volume={4},
    pages={173--186},
    year={2004}
}

@article{li2005mining,
    title={Mining block correlations to improve storage performance},
    author={Li, Zhenmin and Chen, Zhifeng and Zhou, Yuanyuan},
    journal={ACM Transactions on Storage (TOS)},
    volume={1},
    number={2},
    pages={213--245},
    year={2005},
    publisher={ACM}
}

@inproceedings{griffioen1994probabilityGraph,
    title={Reducing File System Latency using a Predictive Approach.},
    author={Griffioen, Jim and Appleton, Randy},
    booktitle={USENIX summer},
    pages={197--207},
    year={1994}
}

@inproceedings{liang2007step,
    title={{STEP}: Sequentiality and thrashing detection based prefetching to improve performance of networked storage servers},
    author={Liang, Shuang and Jiang, Song and Zhang, Xiaodong},
    booktitle={27th International Conference on Distributed Computing Systems (ICDCS'07)},
    pages={64--64},
    year={2007},
    organization={IEEE}
}

@inproceedings{yoon2010intelligent,
    title={Intelligent data prefetching for hybrid flash-disk storage using sequential pattern mining technique},
    author={Yoon, Un-Keun and Kim, Han-joon and Chang, Jae-young},
    booktitle={Computer and Information Science (ICIS), 2010 IEEE/ACIS 9th International Conference on},
    pages={280--285},
    year={2010},
    organization={IEEE}
}


@inproceedings{gu2006nexus,
    title={Nexus: a novel weighted-graph-based prefetching algorithm for metadata servers in petabyte-scale storage systems},
    author={Gu, Peng and Zhu, Yifeng and Jiang, Hong and Wang, Jun},
    booktitle={Cluster Computing and the Grid, 2006. CCGRID 06. Sixth IEEE International Symposium on},
    volume={1},
    pages={8--pp},
    year={2006},
    organization={IEEE}
}


@inproceedings{amer2002group,
    title={Group-based management of distributed file caches},
    author={Amer, Ahmed and Long, Darrell DE and Burns, Randal C},
    booktitle={Distributed Computing Systems, 2002. Proceedings. 22nd International Conference on},
    pages={525--534},
    year={2002},
    organization={IEEE}
}

@phdthesis{Amer:2002:PDG:935782,
    author = {Amer, Ahmed M.},
    title = {Predictive Data Grouping Using Successor Prediction},
    year = {2002},
    isbn = {0-493-81824-3},
    note = {AAI3063076},
    publisher = {University of California, Santa Cruz},
} 

@inproceedings{gopisetty2015support,
    title={Support-Based Prefetching Technique for Hierarchical Collaborative Caching Algorithm to Improve the Performance of a Distributed File System},
    author={Gopisetty, Rathnamma and Ragunathan, T and Bindu, C Shobha},
    booktitle={Parallel Architectures, Algorithms and Programming (PAAP), 2015 Seventh International Symposium on},
    pages={97--103},
    year={2015},
    organization={IEEE}
}


@inproceedings{jeong2015clusterfetch,
    title={ClusterFetch: A Lightweight Prefetcher for General Workloads},
    author={Jeong, Haksu and Ryu, Junhee and Lee, Dongeun and Lee, Jaemyoun and Shin, Heonshik and Kang, Kyungtae},
    booktitle={Proceedings of the 6th ACM/SPEC International Conference on Performance Engineering},
    pages={99--100},
    year={2015},
    organization={ACM}
}

@inproceedings{ryu2015clusterfetch,
    title={ClusterFetch: A Lightweight Prefetcher that Responds to Intensive Disk Read Patterns},
    author={Ryu, Junhee and Jeong, Haksu and Lee, Dongeun and Shin, Heonshik and Kang, Kyungtae},
    booktitle={High Performance Computing and Communications (HPCC), 2015 IEEE 7th International Symposium on Cyberspace Safety and Security (CSS), 2015 IEEE 12th International Conferen on Embedded Software and Systems (ICESS), 2015 IEEE 17th International Conference on},
    pages={1051--1056},
    year={2015},
    organization={IEEE}
}

@inproceedings{jeong2015breakpoint,
    title={Breakpoint-based lightweight prefetching to improve application response},
    author={Jeong, Haegeon and Won, Jiwoong and Lee, Jaemyoun and Kang, Kyungtae and Ryu, Junhee},
    booktitle={Computer Software and Applications Conference (COMPSAC), 2015 IEEE 39th Annual},
    volume={3},
    pages={666--667},
    year={2015},
    organization={IEEE}
}

@inproceedings{lewis2010automatic,
    title={An automatic prefetching and caching system},
    author={Lewis, Joshua and Alghamdi, Mohammed and Al Assaf, Maen and Ruan, Xiaojun and Ding, Zhiyang and Qin, Xiao},
    booktitle={International Performance Computing and Communications Conference},
    pages={180--187},
    year={2010},
    organization={IEEE}
}

@inproceedings{tang2012improved,
    title={An improved adaptive cache prefetch algorithm},
    author={Tang, Limei and Xing, Suxia and Chen, Tianhua},
    booktitle={Computational Intelligence and Design (ISCID), 2012 Fifth International Symposium on},
    volume={2},
    pages={255--258},
    year={2012},
    organization={IEEE}
}

@article{sanders2013real,
    title={Real-time integrated prefetching and caching},
    author={Sanders, Peter and Singler, Johannes and van Stee, Rob},
    journal={Journal of Scheduling},
    volume={16},
    number={1},
    pages={47--58},
    year={2013},
    publisher={Springer}
}

@article{zong2014faststor,
    title={FastStor: improving the performance of a large scale hybrid storage system via caching and prefetching},
    author={Zong, Ziliang and Fares, Ribel and Romoser, Brian and Wood, Joal},
    journal={Cluster Computing},
    volume={17},
    number={2},
    pages={593--604},
    year={2014},
    publisher={Springer}
}


@article{seshadri2015mitigating,
    title={Mitigating prefetcher-caused pollution using informed caching policies for prefetched blocks},
    author={Seshadri, Vivek and Yedkar, Samihan and Xin, Hongyi and Mutlu, Onur and Gibbons, Phillip B and Kozuch, Michael A and Mowry, Todd C},
    journal={ACM Transactions on Architecture and Code Optimization (TACO)},
    volume={11},
    number={4},
    pages={51},
    year={2015},
    publisher={ACM}
}

@inproceedings{Waldspurger2015Shards,
 author = {Waldspurger, Carl A. and Park, Nohhyun and Garthwaite, Alexander and Ahmad, Irfan},
 title = {Efficient MRC Construction with SHARDS},
 booktitle = {Proceedings of the 13th USENIX Conference on File and Storage Technologies},
 series = {FAST'15},
 year = {2015},
 isbn = {978-1-931971-201},
 location = {Santa Clara, CA},
 pages = {95--110},
 numpages = {16},
 url = {http://dl.acm.org/citation.cfm?id=2750482.2750490},
 acmid = {2750490},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 




@article{SNIAMSR, 
 author = {Narayanan, Dushyanth and Donnelly, Austin and Rowstron, Antony},
 title = {Write Off-loading: Practical Power Management for Enterprise Storage},
 journal = {Trans. Storage},
 issue_date = {November 2008},
 volume = {4},
 number = {3},
 month = nov,
 year = {2008},
 issn = {1553-3077},
 pages = {10:1--10:23},
 articleno = {10},
 numpages = {23},
 url = {http://doi.acm.org/10.1145/1416944.1416949},
 doi = {10.1145/1416944.1416949},
 acmid = {1416949},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {DiskEnergy, disk spin-down, energy, enterprise storage, power, write off-loading},
} 


@inproceedings{Koh2005Sporadic,
 author = {Koh, Yun Sing and Rountree, Nathan},
 title = {Finding Sporadic Rules Using Apriori-inverse},
 booktitle = {Proceedings of the 9th Pacific-Asia Conference on Advances in Knowledge Discovery and Data Mining},
 series = {PAKDD'05},
 year = {2005},
 isbn = {3-540-26076-5, 978-3-540-26076-9},
 location = {Hanoi, Vietnam},
 pages = {97--106},
 numpages = {10},
 url = {http://dx.doi.org/10.1007/11430919_13},
 doi = {10.1007/11430919_13},
 acmid = {2140847},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 


@inproceedings{jiang2002LIRS, 
 author = {Jiang, Song and Zhang, Xiaodong},
 title = {LIRS: An Efficient Low Inter-reference Recency Set Replacement Policy to Improve Buffer Cache Performance},
 booktitle = {Proceedings of the 2002 ACM SIGMETRICS International Conference on Measurement and Modeling of Computer Systems},
 series = {SIGMETRICS '02},
 year = {2002},
 isbn = {1-58113-531-9},
 location = {Marina Del Rey, California},
 pages = {31--42},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/511334.511340},
 doi = {10.1145/511334.511340},
 acmid = {511340},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{zhou2001MultiQueue,
 author = {Zhou, Yuanyuan and Philbin, James and Li, Kai},
 title = {The Multi-Queue Replacement Algorithm for Second Level Buffer Caches},
 booktitle = {Proceedings of the General Track: 2001 USENIX Annual Technical Conference},
 year = {2001},
 isbn = {1-880446-09-X},
 pages = {91--104},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=647055.715773},
 acmid = {715773},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 

@inproceedings{Megiddo2003ARC,
 author = {Megiddo, Nimrod and Modha, Dharmendra S.},
 title = {ARC: A Self-Tuning, Low Overhead Replacement Cache},
 booktitle = {Proceedings of the 2Nd USENIX Conference on File and Storage Technologies},
 series = {FAST '03},
 year = {2003},
 location = {San Francisco, CA},
 pages = {115--130},
 numpages = {16},
 url = {http://dl.acm.org/citation.cfm?id=1090694.1090708},
 acmid = {1090708},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 

@inproceedings{Beckmann2015Talus, 
author={N. Beckmann and D. Sanchez}, 
booktitle={2015 IEEE 21st International Symposium on High Performance Computer Architecture (HPCA)}, 
title={Talus: A simple way to remove cliffs in cache performance}, 
year={2015}, 
pages={64-75}, 
keywords={cache storage;Talus;access stream;cache management;cache partitioning;cache performance;cache space;cliff removal;convex fashion;partitioning algorithms;program behavior;single-application performance;Aerospace electronics;Electronics packaging;Hardware;Partitioning algorithms;Quality of service;Resource management;Software}, 
doi={10.1109/HPCA.2015.7056022}, 
ISSN={1530-0897}, 
month={Feb},}


@inproceedings{Narayanan2008MSR,
 author = {Narayanan, Dushyanth and Donnelly, Austin and Rowstron, Antony},
 title = {Write Off-loading: Practical Power Management for Enterprise Storage},
 booktitle = {Proceedings of the 6th USENIX Conference on File and Storage Technologies},
 series = {FAST'08},
 year = {2008},
 location = {San Jose, California},
 pages = {17:1--17:15},
 articleno = {17},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=1364813.1364830},
 acmid = {1364830},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 


@book{han2011dataMiningBook,
  title={Data mining: concepts and techniques},
  author={Han, Jiawei and Pei, Jian and Kamber, Micheline},
  year={2011},
  publisher={Elsevier}
}

@InProceedings{gniady04,
	Author = {Chris Gniady and Ali R. Butt and Y. Charlie Hu},
	Title = {Program-Counter-Based Pattern Classification in Buffer Caching},
	BookTitle = {6th Symp.\ Operating Systems Design \& Implementation (OSDI)},
	Pages = {395--408},
	Month = {Dec},
	Year = {2004},
}


@inproceedings{wong02,
	author = {Wong, Theodore M. and Wilkes, John},
	title = {My Cache or Yours? Making Storage More Exclusive},
	booktitle = {Proceedings of the General Track of the Annual Conference on USENIX Annual Technical Conference},
	series = {ATEC '02},
	year = {2002},
	isbn = {1-880446-00-6},
	pages = {161--175},
	numpages = {15},
	url = {http://dl.acm.org/citation.cfm?id=647057.713858},
	acmid = {713858},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 

@inproceedings{chang99,
	author = {Chang, Fay and Gibson, Garth A.},
	title = {Automatic I/O Hint Generation Through Speculative Execution},
	booktitle = {Proceedings of the Third Symposium on Operating Systems Design and Implementation},
	series = {OSDI '99},
	year = {1999},
	isbn = {1-880446-39-1},
	location = {New Orleans, Louisiana, USA},
	pages = {1--14},
	numpages = {14},
	url = {http://dl.acm.org/citation.cfm?id=296806.296807},
	acmid = {296807},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 

@misc{ioblazer,
  author ={Davide Bergamasco}, 
  title = {IOBLAZER}, 
  howpublished = {\url{https://labs.vmware.com/flings/ioblazer}}, 
  note = {Accessed: 2017-01-30}
}

@inproceedings{Gulati2011Pesto,
 author = {Gulati, Ajay and Shanmuganathan, Ganesha and Ahmad, Irfan and Waldspurger, Carl and Uysal, Mustafa},
 title = {Pesto: Online Storage Performance Management in Virtualized Datacenters},
 booktitle = {Proceedings of the 2Nd ACM Symposium on Cloud Computing},
 series = {SOCC '11},
 year = {2011},
 isbn = {978-1-4503-0976-9},
 location = {Cascais, Portugal},
 pages = {19:1--19:14},
 articleno = {19},
 numpages = {14},
 url = {http://doi.acm.org/10.1145/2038916.2038935},
 doi = {10.1145/2038916.2038935},
 acmid = {2038935},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {QoS, VM, device, modeling, storage, virtualization},
} 

@inproceedings{Tang2015RIPQ,
 author = {Tang, Linpeng and Huang, Qi and Lloyd, Wyatt and Kumar, Sanjeev and Li, Kai},
 title = {RIPQ: Advanced Photo Caching on Flash for Facebook},
 booktitle = {Proceedings of the 13th USENIX Conference on File and Storage Technologies},
 series = {FAST'15},
 year = {2015},
 isbn = {978-1-931971-201},
 location = {Santa Clara, CA},
 pages = {373--386},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=2750482.2750510},
 acmid = {2750510},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 

@inproceedings{vandebogart2009,
  title={Reducing Seek Overhead with Application-Directed Prefetching.},
  author={VanDeBogart, Steve and Frost, Christopher and Kohler, Eddie},
  booktitle={USENIX Annual Technical Conference},
  year={2009}
}

@misc{mimircache,
  author ={Juncheng Yang}, 
  title = {mimircache}, 
  howpublished = {\url{https://github.com/1a1a11a/mimircache}}, 
  note = {Accessed: 2017-01-30}
}

@article{van2009wikibench,
  title={Wikibench: A distributed, wikipedia based web application benchmark},
  author={van Baaren, Erik-Jan},
  journal={Master's thesis, VU University Amsterdam},
  year={2009}
}


@article{Gill2007AMPFull,
 author = {Gill, Binny S. and Bathen, Luis Angel D.},
 title = {Optimal Multistream Sequential Prefetching in a Shared Cache},
 journal = {Trans. Storage},
 issue_date = {October 2007},
 volume = {3},
 number = {3},
 month = oct,
 year = {2007},
 issn = {1553-3077},
 articleno = {10},
 url = {http://doi.acm.org/10.1145/1288783.1288789},
 doi = {10.1145/1288783.1288789},
 acmid = {1288789},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Adaptive prefetching, asynchronous prefetching, cache pollution, degree of prefetch, fixed prefetching, multistream read, optimal prefetching, prefetch wastage, prestaging, sequential prefetching, synchronous prefetching, trigger distance},
} 

@article{spmf2014, 
author = {Fournier-Viger, P. and Gomariz, A. and Gueniche, T. and Soltani, A. and Wu., C. and Tseng, V. S.}, 
journal = {Journal of Machine Learning Research (JMLR)}, 
pages = {3389--3393}, 
title = {{SPMF: a Java Open-Source Pattern Mining Library}}, 
year = {2014}, volume = {15}, url = {http://www.philippe-fournier-viger.com/spmf/} }

